CLOSER: Towards Better Representation Learning for Few-Shot Class-Incremental Learning

Aiming to incrementally learn new classes with only few samples while preserving the knowledge of base (old) classes, few-shot class-incremental learning (FSCIL) faces several challenges, such as overfitting and catastrophic forgetting. Such a challenging problem is often tackled by fixing a feature extractor trained on base classes to reduce the adverse effects of overfitting and forgetting. Under such formulation, our primary focus is representation learning on base classes to tackle the unique challenge of FSCIL: simultaneously achieving the transferability and the discriminability of the learned representation. Building upon the recent efforts for enhancing transferability, such as promoting the spread of features, we find that trying to secure the spread of features within a more confined feature space enables the learned representation to strike a better balance between transferability and discriminability. Thus, in stark contrast to prior beliefs that the inter-class distance should be maximized, we claim that the closer different classes are, the better for FSCIL. The empirical results and analysis from the perspective of information bottleneck theory justify our simple yet seemingly counter-intuitive representation learning method, raising research questions and suggesting alternative research directions. The code is available at https://github.com/JungHunOh/CLOSER_ECCV2024.

==> camera_ready/Figure/visualization.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{submission/Figure/images/cam_visualization_tmp.pdf}
    \caption{\textbf{Visualization of class activation map using \textcolor{black}{Grad-CAM++}~\cite{Chattopadhyay2018gradcampp}.} These examples belong to new classes. Our method correctly predicts the classes, whereas the baseline misclassifies them as base classes.}
    \label{fig:cam}
\end{figure}

==> supple/Figure/intra_inter.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{supple/Figure/images/intra_inter.pdf}
    \caption{\textbf{Comparison between the impact of reducing intra-class and inter-class distance.}
    Reducing intra-class distance harms the performance on new classes (\textcolor{SkyBlue}{dotted sky blue line}) and exacerbates the performance drop from classifier replacement (CR) (\textcolor{violet}{dotted purple line}).
    Conversely, reducing inter-class distance benefits new-class accuracy (\textcolor{SkyBlue}{solid sky blue line}) and alleviates the performance degradation from CR (\textcolor{violet}{solid purple line}).
    The experiments are conducted on CUB200 dataset.
    }
    \label{fig:supp:intra_inter}
\end{figure}

==> supple/Table/intra_inter.tex <==
\begin{table}[t!]
\centering
\small
\caption{\textbf{Comparison between the impact of reducing intra-class and inter-class distance.}
    `Inter-class*' means that the minimization is carried out on a subset of inter-class pairs, which is chosen to have an equal number as the intra-class pairs, ensuring a fair comparison.
    }
\resizebox{0.6\linewidth}{!}{
    \begin{tabular}{lccccc}
      \toprule
      %\multirow{2}{*}{DA.} & \multirow{2}{*}{\textit{low} $\tau$}& \multirow{2}{*}{$\mathcal{L}_{\text{infoNCE}}$} & \multirow{2}{*}{$\mathcal{L}_{cos}$} & \multicolumn{3}{c}{Acc. (\%)} & \multirow{2}{*}{PD. $\downarrow$}\\
      Dataset & Minimization & $A_B$ & $A_N$ & $A_W$ & $A_B^{0,\text{bef}}$-$A_B^{0,\text{aft}}$\\
      \toprule
      \multirow{3}{*}{\small CIFAR100} & Intra-class&68.78&24.30&50.99&2.71\\
      &Inter-class*&70.32&\textbf{27.28}&53.10&\textbf{1.31}\\
      &Inter-class&\textbf{70.72}&27.23&\textbf{53.32}&1.58\\
      \midrule
      \multirow{3}{*}{\small \textit{mini}ImageNet} & Intra-class&71.17&24.10&52.34&0.43\\
      &Inter-class*&71.85&24.48&52.90&0.34\\
      &Inter-class&\textbf{72.03}&\textbf{25.28}&\textbf{53.33}&\textbf{0.21}\\
      \midrule
      \multirow{3}{*}{\small CUB200} & Intra-class&73.12&46.45&59.63&2.58\\
      &Inter-class*&\textbf{76.47}&\textbf{51.47}&\textbf{63.83}&\textbf{0.58}\\
      &Inter-class&76.40&51.06&63.58&0.62\\
      \bottomrule
    \end{tabular}}
    \label{tab:supp:intra_inter}
\end{table}

==> supple/intra_inter.tex <==
\section{Comparison between Reducing Intra-Class and Inter-Class Distance}\label{supp:sec:intra_inter}
As discussed in Section~\textcolor{red}{3.4}, the dispersion of the representations leads to the performance decline in the classifier replacement (CR) process, since it becomes challenging for the class prototype to adequately represent the scattered features via averaging.
One na\"ive solution is to directly suppress the intra-class distribution, which can be implemented by minimizing the intra-class distance:
\begin{equation}
    \mathcal{L}_{\text{intra}} = - \frac{1}{\sum\limits_{i=1}^B \sum\limits_{j>i}^B \mathbbm{1}_{[y_i = y_j]}} \sum\limits_{i=1}^B \sum\limits_{j>i}^B \mathbbm{1}_{[y_i = y_j]} \texttt{sim}(\vz_i,\vz_j).
\end{equation}
However, we find that directly reducing intra-class distance has negative influences on the performance on both base and new classes, as demonstrated in Fig.~\ref{fig:supp:intra_inter} and Table~\ref{tab:supp:intra_inter}.
One possible explanation is that reducing intra-class distribution may adversely affect the representation generalization ability by impeding its capacity to capture fine-grained details among different instances.
This is supported by the largely degraded performance
results presented in both Fig.~\ref{fig:supp:intra_inter} and the results on CUB200 in Table~\ref{tab:supp:intra_inter}, particularly considering the limited number of training examples in CUB200 and its fine-grained-class property.
On the contrary, reducing inter-class distance is observed to achieve outstanding performance both on base and new classes, which validates our assertion on reducing inter-class distance.
%when the distance between classes diminishes, it enables the acquisition of shared information between classes, as a similar concept is discussed in~\cite{zou2022margin} regarding the negative margin in the softmax function.


\input{supple/Figure/intra_inter}
